Experimenting with the p4est library for AMR simulations of two-phase flows

Many physical problems involve spatial and temporal inhomogeneities that require a very fine discretization in order to be accurately simulated. Using an adaptive mesh, a high level of resolution is used in the appropriate areas while keeping a coarse mesh elsewhere. This idea allows to save time and computations, but represents a challenge for distributed-memory environments. The MARS project (for Multiphase Adaptative Refinement Solver) intends to assess the parallel library p4est for adaptive mesh, in a case of a finite volume scheme applied to two-phase flows. Besides testing the library's performances, particularly for load balancing, its user-friendliness in use and implementation are also exhibited here. First promising 3D simulations are even presented.

==> commands.tex <==
% Notations usuelles pour RDS
\def\d{\text{d}}
\newcommand{\Di}{\mathcal{D}_i}
\newcommand{\Dg}{\mathcal{D}_g}
\newcommand{\Dj}{\mathcal{D}_j}
\newcommand{\Dhk}{\mathcal{D}_h^k}
\newcommand{\Ci}{\mathcal{C}_i}
\newcommand{\Cj}{\mathcal{C}_j}
\newcommand{\pCij}{\partial\mathcal{C}_{ij}}
\newcommand{\Cbetai}{\mathcal{C}^{\beta}_i}
\newcommand{\Cun}{\mathcal{C}^1}
\newcommand{\Cinf}{\mathcal{C}^{\infty}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\Mh}{\mathcal{M}_h}
\newcommand{\Mhstar}{\Mh^*}
\renewcommand{\phi}{\varphi}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\phiit}{\phi_i^{\T}}
\newcommand{\phiik}{\phi_i^k}
\newcommand{\phii}{\phi_i}
\newcommand{\phiij}{\phi_i^j}
\newcommand{\phit}{\phi^{\T}}
\newcommand{\phiE}{\phi_{\Elmt}}
\newcommand{\PhiiEtoile}{\Phi_i^{*}}
\newcommand{\Phiit}{\Phi_i^{\T}}
\newcommand{\Phii}{\Phi_i}
\newcommand{\Phit}{\Phi^{\T}}
\newcommand{\Thetait}{\Theta_i^{\T}}
\newcommand{\Bit}{\beta_i^{\T}}
\newcommand{\BitEtoile}{\beta_i^{\T,*}}
\newcommand{\BiEtoile}{\beta_i^{*}}
\newcommand{\xit}{\xi_i^{\T}}
\newcommand{\x}{\boldsymbol{\vec{x}}}
\newcommand{\m}{n} %\boldsymbol{n}}
\renewcommand{\u}{\vect{u}}
\renewcommand{\v}{\boldsymbol{\vec{v}}}
\renewcommand{\c}{\boldsymbol{\vec{c}}}
\newcommand{\redv}{\Magenta{\boldsymbol{\vec{v}}}}
\newcommand{\redc}{\Magenta{\boldsymbol{\vec{c}}}}
\newcommand{\redu}{\Magenta{\boldsymbol{\vec{u}}}}
\newcommand{\Force}{\boldsymbol{\vec{\text{F}}}}
\newcommand{\SSigma}{\VertECP{{\Sigma}}}
\newcommand{\Chi}{\boldsymbol{\chi}}
%\newcommand{\Upsilon}{\boldsymbol{\upsilon}}
\newcommand{\uinp}{u_i^{n+1}}
\newcommand{\uin}{u_i^{n}}
\newcommand{\U}{{\bf U}}
\newcommand{\Uhat}{\hat{\U}}
\newcommand{\Ui}{\U_i}
\newcommand{\Uj}{\U_j}
\newcommand{\Uinp}{\U_i^{n+1}}
\newcommand{\Uin}{\U_i^{n}}
\newcommand{\W}{\vect{W}}
\newcommand{\What}{\hat{\W}}
\newcommand{\Wstar}{\W^*}
\newcommand{\Wi}{\W_i}
\newcommand{\Wbari}{\overline{\W}_i}
\newcommand{\WbarT}{\overline{\W}_\T}
\newcommand{\Wj}{\W_j}
\newcommand{\Wij}{\W_i^j}
\newcommand{\Winp}{\W_i^{n+1}}
\newcommand{\Win}{\W_i^{n}}
\newcommand{\ctilde}{\tilde{c}_{ij}}
\newcommand{\psiit}{\Psi_i^{\T}}
\newcommand{\gT}{\gamma^{\T}}
\newcommand{\giT}{\gamma_i^{\T}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\G}{\mathcal{G}}
\renewcommand{\H}{\mathcal{H}}
\newcommand{\Flux}{\text{F}}
\newcommand{\Glux}{\text{G}}
\newcommand{\Hlux}{\text{H}}
\newcommand{\Fstar}{\F^*}
\newcommand{\Fh}{\F_h}
\newcommand{\FhUb}{\Fh \left(\U_{\text{bound}}\right)}
\newcommand{\Fub}{\F \left(u_{\text{bound}}\right)}
\newcommand{\V}{{\bf V}}
\newcommand{\X}{{\bf X}}
\newcommand{\Xhat}{\widehat{\X}} 
\newcommand{\xhat}{\widehat{\x}}
\newcommand{\demi}{\frac{1}{2}}
\newcommand{\xipdemi}{x_{i+\demi}} 
\newcommand{\ximdemi}{x_{i-\demi}}
\newcommand{\Fipdemi}{\F^*_{i+\demi}} 
\newcommand{\Fimdemi}{\F^*_{i-\demi}} 
\newcommand{\D}{{\bf D}}
\newcommand{\n}{\vec{\bf n}}
\newcommand{\niT}{\n_i^\T}
\newcommand{\nSF}{\overrightarrow{\textbf{n}_{\text{S}\rightarrow\text{F}}}}
\newcommand{\nij}{\n_{ij}}
\newcommand{\dy}{\vec{\bf dy}}
\newcommand{\barn}{\bar{\bf n}}
\newcommand{\barf}{\bar{f}}
\newcommand{\barrho}{\overline{\rho}}
\newcommand{\tildeRho}{\tilde{\rho}}
\newcommand{\ugbar}{\overline{\boldsymbol{u_g}}}
\newcommand{\ug}{\bf u_g}
\newcommand{\ugprime}{\bf u_g'}
\newcommand{\ui}{\vec{\bf u}_i}
\newcommand{\uwall}{\u_{\text{wall}}}
%\renewcommand{\vecv}{\vec{\bf v}}
\newcommand{\q}{\vec{\bf q}}
\newcommand{\Deformation}{\mathbb{D}}
\newcommand{\viscous}{\mathbb{T}}%\bbtau}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\Aronde}{\mathcal{A}}
\newcommand{\opD}{\mathcal{D}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\RMat}{\mathcal{R}}
\newcommand{\MMat}{\mathcal{M}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\Lun}{\L^1}
\newcommand{\Lde}{\L^2}
\newcommand{\Linfty}{\L^{\infty}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\blambda}{\textcolor{Bleu}{\boldsymbol{\lambda}}}
\newcommand{\bmu}{\textcolor{VertECP}{\boldsymbol{\mu}}}
\newcommand{\vblambda}{\vec{\boldsymbol{\lambda}}}
\newcommand{\bphi}{\boldsymbol{\varphi}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\aireT}{\lvert \T \rvert}
\newcommand{\aireDi}{\lvert \Di \rvert}
\newcommand{\aireCi}{\lvert \Ci \rvert}
\newcommand{\alphaT}{\alpha^\T}
\newcommand{\unzero}{{\vert (\u.\n=0)}}
\newcommand{\usn}{\u.\n}


\newcommand{\ueps}{u_{\varepsilon}}
\newcommand{\Gbf}{\textbf{G}}
\newcommand{\Fbf}{\textbf{F}}
\newcommand{\K}{\mathscr{K}}
\newcommand{\BubbleNi}{\mathscr{N}_i^{\T}}
\newcommand{\Norm}[2]{\lVert #1 \rVert_{#2}}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\Trace}[1]{\text{\bf Tr}\left( #1 \right)}
\newcommand{\Ec}{\mathscr{E}_c}
\newcommand{\enthalpie}{\mathcal{H}}
\newcommand{\HFV}{\overrightarrow{\boldsymbol{\mathcal{H}}}}
\newcommand{\un}{\u.\n}
\newcommand{\E}{\mathscr{E}}
\newcommand{\Eh}{\mathscr{E}_h}
\newcommand{\Elmt}{\mathcal{E}}
\newcommand{\Lronde}{\mathscr{L}}
\newcommand{\diamomd}{\Diamond}
\newcommand{\ustar}{u^{*}}
\newcommand{\Wh}{\W_h}
\newcommand{\ixhk}{\mathscr{X}_h^k}
\newcommand{\Ph}{\mathcal{P}_h}
\newcommand{\Vh}{\mathcal{V}_h}
\newcommand{\Th}{\mathcal{T}_h}
\newcommand{\ds}{\displaystyle}
\renewcommand{\th}{^{\text{th}}}
\newcommand{\nd}{^{\text{nd}}}
\newcommand{\rd}{^{\text{rd}}}
\newcommand{\ndofs}{n_{\text{DoFs}}}
\newcommand{\nV}{n_{\text{V}}}
\newcommand{\nE}{n_{\text{E}}}
\newcommand{\et}{\; \text{ and } \; }
\newcommand{\dxhat}{d\xhat}
\newcommand{\dX}{d\boldsymbol{X}}
\newcommand{\dt}{\Delta t}
\newcommand{\dxmin}{\Delta x_{\text{min}}}
\newcommand{\dxmax}{\Delta x_{\text{max}}}

%\newcommand{\Pr}{Pr}


% Customisation de commandes deja existantes
\newcommand{\dd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\DD}[2]{\dfrac{\D #1}{\D #2}}
\newcommand{\Vect}[1]{\overrightarrow{#1}}
\newcommand{\Div}[1]{\Vect{\nabla} . #1}
%\renewcommand{\div}[1]{\text{div}\left(#1\right)}
\newcommand{\Int}{\displaystyle \int}
\newcommand{\Sum}{\displaystyle \sum}
\newcommand{\tw}{\textwidth}
\renewcommand{\th}{\textheight}
\newcommand{\lw}{\linewidth}
\newcommand{\eq}{\Leftrightarrow}

% Ensembles
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Qu}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Pet}{\mathbb{P}}
\newcommand{\IK}{\mathbb{K}}
\newcommand{\Qun}{\Qu^1}
\newcommand{\Qk}{\Qu^k}
\newcommand{\Ess}{\mathcal{S}}
\newcommand{\Hronde}{\mathcal{H}}
\newcommand{\Fluid}{\Omega_{\text{F}}}
\newcommand{\Struct}{\Omega_{\text{S}}}
\newcommand{\GammaS}{\Gamma_{\text{S}}}
\newcommand{\GammaCV}{\Gamma_{\text{CV}}}
\newcommand{\GammaRec}{\Gamma_{\text{Rec}}}


% Forcer le mode texte
\newcommand{\T}{\text{T}}
\newcommand{\Kmat}{\textbf{K}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\I}{\textbf{I}}
\newcommand{\Iij}{\text{I}_{ij}}
%\renewcommand{\l}{l}
\newcommand{\Q}{\text{Q}}
\newcommand{\Qhat}{\widehat{\Q}}
\newcommand{\A}{\text{A}}
\newcommand{\B}{\text{B}}
\newcommand{\MatC}{\text{C}}
\newcommand{\divergence}[1]{\text{div}\left(#1\right)}
\newcommand{\Szero}{\text{S}_0}
\newcommand{\Pxi}{\text{P}(\bxi)}
\newcommand{\PNoir}{\mathbb{P}}
\renewcommand{\P}{\textcolor{red}{\mathbb{P}}}
\newcommand{\EtotNoir}{\mathbb{E}}
\newcommand{\Etot}{\textcolor{DarkGreen}{\mathbb{E}}}
\newcommand{\Sym}{\ocirc}
\newcommand{\PScal}{\textcolor{red}{p}}
\newcommand{\EtotScal}{\textcolor{DarkGreen}{\boldsymbol{E}}}
\newcommand{\SymScal}{\cdot}
\newcommand{\otimesScal}{\cdot}
\newcommand{\Dxi}{\text{D}(\bxi)}
\newcommand{\Qxi}{\text{Q}(\bxi)}
\newcommand{\trans}{\text{T}}
\newcommand{\SphereD}{\text{S}^{d-1}}
\newcommand{\CFD}{\text{CFD}}
\newcommand{\PDE}{\text{PDE}}
\newcommand{\PDS}{\text{PDS}}
\newcommand{\chara}{\textit{Char}}
\newcommand{\dof}{\text{DoF}}
\newcommand{\dofs}{\text{DoF}s}
\newcommand{\Qronde}{\mathscr{Q}}
\newcommand{\Qrhat}{\widehat{\Qronde}}
\newcommand{\Qi}{\Qronde_i}
\newcommand{\intermediaire}{\text{D}}
\newcommand{\edge}{\text{edge}}
\newcommand{\nedge}{\n_\edge}
\newcommand{\lrond}{\mathit{l}}
\newcommand{\quadrature}{\text{quad}}
\newcommand{\slip}{\text{slip}}
\newcommand{\IB}{\text{IB}}
\newcommand{\chii}{\chi_i}
\renewcommand{\Re}{\text{Re}}
\newcommand{\Ma}{\text{Ma}}
%\newcommand{\det}{\text{det}}


% Raccourcis bien pratiques
\newcommand{\vki}{von Karman Institute for Fluid Dynamics}
\newcommand{\FdB}{FluidBox}
\newcommand{\eg}{\textit{e.g. }}
\renewcommand{\ae}{\textit{a.e. }}
\newcommand{\aso}{\textit{aso... }}
\renewcommand{\emph}{\textit}

% Methodes
\newcommand{\LxF}{\text{LxF}}
\newcommand{\EOS}{\text{EOS}}
\newcommand{\FSI}{\text{FSI}}
\newcommand{\ROE}{\text{ROE}}
\newcommand{\CPU}{\text{CPU}}
\newcommand{\LLxF}{\text{LLxF}}
\newcommand{\LP}{$\mathcal{LP}$}
\newcommand{\RD}{$\mathcal{RD}$}
\newcommand{\RDS}{$\mathcal{RDS}$}
\newcommand{\MHD}{\text{MHD}}
\newcommand{\RHS}{$\mathcal{RHS}$}
\newcommand{\DG}{$\mathcal{DG}$}
\newcommand{\FV}{$\mathcal{FV}$}
\newcommand{\LW}{$\mathcal{LW}$}
\newcommand{\FE}{$\mathcal{FE}$}
\newcommand{\FS}{$\mathcal{FS}$}
\newcommand{\PG}{$\mathcal{PG}$}
\newcommand{\CL}{$\mathcal{CL}$}


%macros
\newcommand{\mean}[1]{\underline{#1}}

\def\evap{\mathrm{R_S}}
\def\Ev{\mathrm{E\scriptstyle{v}}}
\def\bx{\mathbf{x}}
\def\bu{\mathbf{u}}
\def\bn{\mathbf{n}}
\def\be{\mathbf{e}}
\def\bU{\mathbf{U}}
\def\bF{\mathbf{F}}
\def\bg{\mathbf{g}}
\newcommand{\bfGamma}{\text{\boldmath $\Gamma$}}
\newcommand{\bfgamma}{\text{\boldmath $\gamma$}}
\newcommand{\bfLambda}{\text{\boldmath $\Lambda$}}
\newcommand{\bfxi}{\text{\boldmath $\xi$}}
\newcommand{\bfeta}{\text{\boldmath $\eta$}}
\newcommand{\bfzeta}{\text{\boldmath $\zeta$}}
\newcommand{\bfvarphi}{\text{\boldmath $\varphi$}}
\newcommand{\bfepsilon}{\text{\boldmath $\epsilon$}}
\newcommand{\bfF}{\text{${\bf F}$}}
\newcommand{\bfE}{\text{${\bf E}$}}
\newcommand{\bfX}{\text{${\bf X}$}}
\newcommand{\luiujr}{\text{$\langle u_iu_j \rangle$}}
\newcommand{\bfn}{\text{${\bf n}$}}
%\newcommand{\bfc}{\text{${\bf c}$}}
\newcommand{\bfx}{\text{${\bf x}$}}
\newcommand{\bfq}{\text{${\bf q}$}}
\newcommand{\vbfxt}{\text{$\varepsilon({\bf x},t)$}}
\newcommand{\bfxt}{\text{$({\bf x},t)$}}
\newcommand{\bfpsi}{\text{\boldmath $\psi$}}
\newcommand{\bfPhi}{\text{\boldmath $\Phi$}}
\newcommand{\bftheta}{\text{\boldmath $\theta$}}
\newcommand{\bfmu}{\text{\boldmath $\mu$}}
\newcommand{\Pijstar}{\text{$Pi_{ij}^*$}}
\newcommand{\p}{\text{$\partial$}}
\newcommand{\bfa}{\text{${\bf a}$}}
\newcommand{\bfk}{\text{${\bf k}$}}
\newcommand{\bfW}{\text{${\bf W}$}}
\newcommand{\bfD}{\text{${\bf D}$}}
\newcommand{\bfA}{\text{${\bf A}$}}
\newcommand{\bfu}{\text{${\bf u}$}}
\newcommand{\bfz}{\text{${\bf z}$}}
\newcommand{\bfB}{\text{${\bf B}$}}
\newcommand{\bfC}{\text{${\bf C}$}}
\newcommand{\bfR}{\text{${\bf R}$}}
\newcommand{\bfQ}{\text{${\bf Q}$}}
\newcommand{\bfw}{\text{${\bf w}$}}
\newcommand{\bfr}{\text{${\bf r}$}}
\newcommand{\bfP}{\text{${\bf P}$}}
\newcommand{\bfL}{\text{${\bf L}$}}
\newcommand{\rT}{\text{T}}
\newcommand{\bfnabla}{\text{\boldmath $\nabla$}}
\newcommand{\bfalpha}{\text{\boldmath $\alpha$}}
\newcommand{\bfdelta}{\text{\boldmath $\delta$}}
\newcommand{\bfnu}{\text{\boldmath $\nu$}}
\newcommand{\bfchi}{\text{\boldmath $\chi$}}
\newcommand{\bfb}{\text{${\bf b}$}}
\newcommand{\bfc}{\text{${\bf c}$}}
\newcommand{\bfd}{\text{${\bf d}$}}
\newcommand{\bfe}{\text{${\bf e}$}}
\newcommand{\bff}{\text{${\bf f}$}}
\newcommand{\bfg}{\text{${\bf g}$}}
\newcommand{\bfh}{\text{${\bf h}$}}
\newcommand{\bfone}{\text{${\bf 1}$}}
\newcommand{\bfS}{\text{${\bf S}$}}
\newcommand{\bfT}{\text{${\bf T}$}}
\newcommand{\bfM}{\text{${\bf M}$}}
\newcommand{\bfU}{\text{${\bf U}$}}
\newcommand{\bfV}{\text{${\bf V}$}}
\newcommand{\bfs}{\text{${\bf s}$}}
\newcommand{\bfy}{\text{${\bf y}$}}
\newcommand{\bfI}{\text{${\bf I}$}}
\newcommand{\diag}{\text{${\bf diag}$}}
\newcommand{\bftau}{\text{\boldmath ${\bf \tau}$}}
\newcommand{\bfrho}{\text{\boldmath ${\bf \rho}$}}
\newcommand{\bfzero}{\text{\boldmath ${\bf 0}$}}
\newcommand{\bfomega}{\text{\boldmath ${\bf \omega}$}}
\newcommand{\bfvarepsilon}{\text{\boldmath ${\bf \varepsilon}$}}
\newcommand{\bfv}{\text{\boldmath ${\bf v}$}}
\newcommand{\phiprime}{\text{${\phi'}$}}
\newcommand{\bfphiprime}{\text{\boldmath ${\phi'}$}}
\newcommand{\bfphi}{\text{\boldmath ${\phi}$}}
\newcommand{\sd}{\text{${\, \rm d}$}}
\newcommand{\rD}{\text{${\rm D}$}}
\newcommand{\lbfsr}{\text{$\langle \bfs\rangle$}}
\newcommand{\lbfphir}{\text{$\langle \bfphi\rangle$}}
\newcommand{\lxir}{\text{$\langle \xi\rangle$}}
\newcommand{\Moment}{\mathcal{M}}

%%% Color Commands for presentations
\definecolor{DarkGreen}{rgb}{0.,0.5,0.}
\definecolor{Bordeaux}{rgb}{0.75,0.,0.}
\definecolor{AppleGreen}{rgb}{0.,0.75,0.}
\definecolor{orange}{rgb}{0.97,0.65,0.02}
\definecolor{purple}{rgb}{0.61,0,0.99}
\definecolor{pink}{rgb}{0.98,0,0.99}

\newcommand{\Red}[1]{\textcolor{red}{#1}}
\newcommand{\VertECP}[1]{\textcolor{VertECP}{#1}}
\newcommand{\Magenta}[1]{\textcolor{Magenta}{#1}}
\newcommand{\Bleu}[1]{\textcolor{Bleu}{#1}}
\newcommand{\Pomme}[1]{\textcolor{Pomme}{#1}}
\newcommand{\Orange}[1]{\textcolor{Orange}{#1}}
\newcommand{\Purple}[1]{\textcolor{purple}{#1}}
\newcommand{\Pink}[1]{\textcolor{pink}{#1}}
\newcommand{\St}{St}

\newcommand{\adam}[1]{\textcolor{red}{Ad.: \textbf{#1}}}
\newcommand{\maldit}[1]{\textcolor{red}{\textit{#1}}}

\newcommand{\beq}[1]{\begin{equation}\label{#1}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bitem}{\begin{itemize}}
\newcommand{\eitem}{\end{itemize}}

